Finding Skewed Subcubes Under a Distribution

Say that we are given samples from a distribution $\psi$ over an $n$-dimensional space. We expect or desire $\psi$ to behave like a product distribution (or a $k$-wise independent distribution over its marginals for small $k$). We propose the problem of enumerating/list-decoding all large subcubes where the distribution $\psi$ deviates markedly from what we expect; we refer to such subcubes as skewed subcubes. Skewed subcubes are certificates of dependencies between small subsets of variables in $\psi$. We motivate this problem by showing that it arises naturally in the context of algorithmic fairness and anomaly detection. In this work we focus on the special but important case where the space is the Boolean hypercube, and the expected marginals are uniform. We show that the obvious definition of skewed subcubes can lead to intractable list sizes, and propose a better definition of a minimal skewed subcube, which are subcubes whose skew cannot be attributed to a larger subcube that contains it. Our main technical contribution is a list-size bound for this definition and an algorithm to efficiently find all such subcubes. Both the bound and the algorithm rely on Fourier-analytic techniques, especially the powerful hypercontractive inequality. On the lower bounds side, we show that finding skewed subcubes is as hard as the sparse noisy parity problem, and hence our algorithms cannot be improved on substantially without a breakthrough on this problem which is believed to be intractable. Motivated by this, we study alternate models allowing query access to $\psi$ where finding skewed subcubes might be easier.

==> skew.tex <==
\subsection*{Skew}

\begin{definition}[Skew]
	We define the \textbf{skew} of a subcube $C$ with respect to measure $\psi$ as
	\[ \skew_\psi(C) = \ip{\psi, \mu_C} - 1\]
\end{definition}

We give two convenient characterizations of skew.

\begin{Lem}
	\label{lem:skew_by_prob}
  Let $\codim(C) = k$. We have
  \begin{align*}
  \skew_\psi(C) &= 2^k \left(\Pr_{x \sim \psi}[\x \in C] - \Pr_{x
    \sim \mu}[\x \in C] \right) \\
	&= \sum_{\emptyset \neq S \subseteq
	K} \hatpsi(S)\chi_S(y)
  \end{align*}
\end{Lem}
\begin{proof}
  We have
\begin{align*}
  \ip{\psi, \mu_C} & = \E_{\x \in C}[\psi(\x)]\\
  & = \sum_{x \in C}\frac{\psi(\x)}{2^{n-k}}\\
  & = 2^k \sum_{x \in C}\Pr_{\x \sim \psi}[\x =x]\\
  & = 2^k \Pr_{\x \sim \psi}[\x \in C].
\end{align*}
Since $\Pr_{\x \sim \mu}[\x \in C] = 2^{-k}$, the first equality follows. To see the second:

\end{proof}

We show that the existence of negatively skewed subcubes also implies the existence of positively skewed cubes.

\begin{Lem}
	\label{lem:chainrule}
	For $\gamma > 0$, if subcube $C = (K, y)$ has $\skew(C) = -\gamma$, then
        there exists a $y' \in \pmo^K$ such that $C' = (K, y')$ has
        $\skew(C') \geq \gamma/2^{|K|}$.
\end{Lem}

\begin{proof}
	Consider the sum:
	\begin{align*}
	\sum_{\substack{D = (K, w) \\ w \in \pmo^K}} \skew(D) =
        \sum_{\substack{D = (K, w) \\ w \in \pmo^K}} 2^k \left(\Pr_{x
          \sim \psi}[\x \in D] - \Pr_{x \sim \mu}[\x \in D] \right) =
        0.
	\end{align*}
	The first equality comes from \cref{lem:skew_by_prob}, the
        second follows since the set of cubes $D$ form a partition of
        $\pmo^n$. Since there are $2^{|K|}$ terms in the sum above,
        for at least one $y' \in \pmo^K$ it is the case that $C' = (K,
        y')$ has $\skew(C') \geq -\skew(C)/2^{|K|}$.
\end{proof}


\begin{Lem}
\label{lem:comb_lb}
  For any $0 \leq \gamma \leq 2^k -1$, there exists a distribution
  $\psi$ such that there are $\Omega((n/k)^k)$ many $\gamma$-skewed
  subcubes of codimension $k$.
\end{Lem}
\begin{proof}
  Set $f = \lceil \log_2(1 + \gamma) \rceil$.
  Let $C$ be the subcube where the first $t \geq f$ bits are fixed to $1$, and let $\mu_C$ be the uniform distribution over it.
  Consider any subcube $D$ where we choose $f$ indices from $[t]$ and $k - f$ indices from $[n]
  \setminus [t]$, and set them to $1$.
  We have
  \begin{align*}
    \ip{\mu_C, \mu_D} & = \E_{\mu_C}[\mu_D]  = 2^k\Pr_{\x \sim \mu_C}[\x \in D]
    = 2^k\frac{1}{2^{k -f}} = 2^f \geq 1 + \gamma
  \end{align*}
since a point from $\mu_C$ lies in $D$ iff the $k -f$ bits from
$[n]\setminus [t]$ are all set to $1$. We now optimize the choice of
$t$. Let $f = \alpha k$ for $\alpha \leq 1$. We choose $t = \alpha n$
(ignoring floors and ceilings which wont affect the asymptotics). The
number of choices for $D$ is given by
\[ \binom{t}{f}\cdot \binom{n -t}{k -f}  = \binom{\alpha n}{\alpha
  k}\cdot \binom{(1- \alpha)n}{(1 - \alpha)k} \geq
  \left(\frac{n}{k}\right)^{\alpha k}\cdot \left(\frac{n}{k}\right)^{(1
    - \alpha)k} \geq  \left(\frac{n}{k}\right)^k. \]
\end{proof}

Given that this bound is not too far from the trivial upper bound of
$\binom{n}{k}$, we need to refine our notion of skew, and also to
restrict the set of distributions we consider. First we only
consider {\em well-spread} distributions where $\inorm{\psi}$ is
bounded. Secondly, we discount subcubes that inherit their skew from
their parent subcubes.

Given a cube $C = (K, y)$ of codimension $k$, we can partition it into
$2^\ell$ subcubes of codimension $k + \ell$, where we pick a set $L$ of $\ell$
additional coordinates outside of $K$ to fix and enumerate over all
settings of these coordinates.

\begin{Lem}
\label{lem:skew_avg}
  If $\{C_1, \ldots, C_{2^\ell}\}$ is a partition of $C$, then
  \[ \skew_\psi(C) = \frac{1}{2^\ell}\sum_{i=1}^{2^\ell}\skew_\psi(C_i). \]
\end{Lem}
\begin{proof}
  We have
\begin{align*}
    \skew_\psi(C) & = 2^k\left(\Pr_{\x \sim \psi}[\x \in C ] - \frac{1}{2^k}\right)\\
      & = \frac{2^{k+ \ell}}{2^\ell}\left(\sum_{i=1}^{2^\ell}\left(\Pr_{\x \sim \psi}[\x \in C_i] - \frac{1}{2^{k+
        \ell}}\right)\right)\\
      & = \frac{1}{2^\ell}\left(\sum_{i=1}^{2^\ell}2^{k + \ell}\left(\Pr_{\x \sim \psi}[\x \in C_i] - \frac{1}{2^{k+
        \ell}}\right)\right)\\
     & = \frac{1}{2^\ell}\sum_{i=1}^{2^\ell} \skew_\psi(C_i)
\end{align*}
\end{proof}

An implication is that there exists $C$ such that $\codim(C) = k -
\ell$ and $\skew(C) \geq \gamma$, then there exist $\binom{n -k +
  \ell}{\ell}$ subcubes $D$ of $C$ with $\codim(D) = k$ and $\skew(D)
\geq \gamma$. This suggests that we ought to ignore subcubes that can
be viewed as {\em inheriting} skew from their parents, and instead
focus on subcubes whose skew is greater than any parent. This
motivates the following definition:

\begin{definition}
Let $\gamma \in(0,2^k -1]$ and $\eps \in (0,1]$. A subcube $C \subseteq \pmo^n$ is an $(\gamma, \eps)$-minimal
  skewed subcube if $\skew(C) \geq \gamma$ and for all its parent
  subcubes $D \supsetneq C$, we have
  \begin{align}
    \label{eq:min_skew}
    \skew_\psi(D) \leq (1 - \eps)\gamma.
  \end{align}
\end{definition}

The following structural lemma shows that minimal skew cannot be
inherited from a parent. Given a minimal skewed subcube $C$, and a
parent $D \supsetneq C$, the following lemma shows that $C$ has noticeable skew in the
restriction $\restr{\psi}{D}$. This is in constrast to the case of
minimal subsubes, where the skew of $C$ might not be large, once we
restrict the distribution to $D$. This will be
crucial to being able to bound their number and find them
algorithmically.

\begin{Lem}
\label{lem:cond_skew}
  Let $C$ be a $(\gamma, \eps)$-minimal skewed subcube.
  If $D \supseteq C$ is a parent of $C$, then
  \[ \skew_{\restr{\psi}{D}}(C) \geq \frac{\eps \sqrt{\gamma}}{2}. \]
\end{Lem}
\begin{proof}
  By Lemma \ref{lem:prod_rule}
  \begin{align*}
    \ip{\restr{\psi}{D}, \restr{\mu_C}{D}}  & =
    \frac{\ip{\psi, \mu_C}}{\ip{\psi, \mu_D}}\\
    & = \frac{1 + \skew_\psi(C)}{1 + \skew_\psi(D)}\\
    &\geq \frac{1 + \gamma}{ 1 + (1 - \eps)\gamma}
  \end{align*}
  We have
  \begin{align*}
    \skew_{\restr{\psi}{D}}(C) &= \ip{\restr{\psi}{D},
      \restr{\mu_C}{D}} - 1 \\
    & \geq \frac{1 + \gamma}{ 1 + (1 - \eps)\gamma} -1\\
    & = \frac{\eps\gamma}{1 + (1 - \eps)\gamma}\\
    & \geq  \frac{\eps\gamma}{2\sqrt{(1 - \eps)\gamma}}\\
    & \geq \frac{\eps \sqrt{\gamma}}{2}
  \end{align*}
  where the second inequality is by the AM-GM inequality.
\end{proof}

